Understanding Reentrance in Frustrated Magnets: the Case of the Er$_2$Sn$_2$O$_7$ Pyrochlore

Reentrance, the return of a system from an ordered phase to a previously encountered less-ordered one as a controlled parameter is continuously varied, is a recurring theme found in disparate physical systems, from condensed matter to black holes. While diverse in its many incarnations and generally unsuspected, the cause of reentrance at the microscopic level is often not investigated thoroughly. Here, through detailed characterization and theoretical modeling, we uncover the microscopic mechanism behind reentrance in the strongly frustrated pyrochlore antiferromagnet Er$_2$Sn$_2$O$_7$. Taking advantage of the recent advance in rare earth stannate single crystal synthesis, we use heat capacity measurements to expose that Er$_2$Sn$_2$O$_7$ exhibits multiple instances of reentrance in its magnetic field $B$ vs. temperature $T$ phase diagram for magnetic fields along three cubic high symmetry directions. Through classical Monte Carlo simulations, mean field theory and classical linear spin-wave expansions, we argue that the origins of the multiple occurrences of reentrance observed in Er$_2$Sn$_2$O$_7$ are linked to soft modes. Depending on the field direction, these arise either from a direct $T=0$ competition between the field-evolved ground states, or from a field-induced enhancement of the competition with a distinct zero-field antiferromagnetic phase. In both scenarios, the phase competition enhances thermal fluctuations which entropically stabilize a specific ordered phase. This results in an increased transition temperature for certain field values and thus the reentrant behavior. Our work represents a detailed examination into the mechanisms responsible for reentrance in a frustrated magnet and may serve as a template for the interpretation of reentrant phenomena in other physical systems.

==> MonteCarlo.tex <==
\section{Monte Carlo simulations and Parameters}
\label{SM-MC}


Monte Carlo simulations are performed on systems of classical Heisenberg spins with $N=16L^{3}$ sites, where $L^{3}$ is the number of cubic unit cells. The spin length is $|S|=1/2$. Several update algorithms are used together: the heatbath method, over-relaxation and parallel tempering. Parallel tempering is done every 100 Monte Carlo steps (MCS) and overrelaxation is done at every MCS. Thermalization is made in two steps: first a slow annealing from high temperature to the temperature of measurement $T$ during $t_{e}$ MCS followed by $t_{e}$ MCS at temperature $T$. After thermalization, measurements are done every 10 MCS during $t_{m}=10~t_{e}$ MCS.

The characteristics of our simulations are typically:
\begin{itemize}
    \item $4 < L < 10$,
    \item $10^6 \leq t_{m} \leq 5. 10^7$ MCS,
    \item 100 different temperatures (regularly spaced) between 0 and 200 mK for parallel tempering.
\end{itemize}

Please note that different exchange parameters for \ESO\ have been investigated, within the error bars of  Ref.~\cite{ESOPetitPRL}. In particular, a systematic search in the [111] direction has shown a consistent increase of the transition temperature between 0 and 0.4 T, confirming the robustness of the reentrance in this exchange-parameter region.

==> MonteCarloField.tex <==
\section{Monte Carlo simulations at low field in the [110] direction}
\label{SM-Analysis110MCsmallfield}


\begin{figure}[ht]
\centering\includegraphics[width=17cm]{Images/paperESOPClowh.pdf}
\caption{
At low field in the $[110]$ direction, there are four FEPC ground states $\{\langle xz \rangle_h, \langle yz \rangle_h, \langle \overline{xz} \rangle_h, \langle \overline{yz} \rangle_h\}$ and two FEPC excited states $\{\langle xy \rangle_h, \langle \overline{xy} \rangle_h\}$ [see Fig.~\ref{fig:VMFTResults}]. The very small energy gap between them means that it is not obvious which order is stabilised at finite temperature.\\
The easiest way to differentiate between the ground and excited states in Monte Carlo simulations is via the $z$-component of the Palmer-Chalker order parameter, $m_{\rm PCz}$ [see (a,b,c) panels]. $m_{\rm PCz}$ is finite for the two excited states, while it is zero for the four ground states. Here we show that as the system size is increased, $m_{\rm PCz}$ vanishes for $B=$ 0.1 and 0.15 T, which means the FEPC excited states are not stable for $B\gtrsim 0.1$ T. For $B=$ 0.05 T on the other hand, simulations are difficult to thermalize and the evolution with system size is not monotonic. Hence, we cannot rule out the presence of the FEPC excited states at finite temperature, as predicted by mean field theory in the previous section. That being said, this possible co-existence would only arise at very low field, $B\lesssim 0.1$ T, and thus not affect the mechanism for reentrance.\\
As for the four FEPC ground states, they can be divided into two pairs. For $\langle \overline{xz} \rangle_h$ and $\langle \overline{yz} \rangle_h$, the $x$-component of the Palmer-Chalker order parameter is positive, $m_{\rm PCx}>0$. For $\langle xz \rangle_h$ and $\langle yz \rangle_h$, $m_{\rm PCx}<0$. As shown in panels (d,e,f), $m_{\rm PCx}$ always gets more and more positive for large system sizes, which means that the Z$_{2}$ states at low $[110]$ field are $\langle \overline{xz} \rangle_h$ and $\langle \overline{yz} \rangle_h$. At very low temperatures, $T< 40$ mK, the data split into two groups because of the broken ergodicity in simulations between $\langle \overline{xz} \rangle_h$ and $\langle \overline{yz} \rangle_h$.\\
All of these simulations were done for $t_{m}=5. 10^{7}$ Monte-Carlo steps.
}
\label{fig:110PCSM}
\end{figure}
%------------------------------------------------------------------------
\clearpage


\section{Monte Carlo simulations in the [111] direction}
\label{SM-Analysis111MC}


\begin{figure}[ht]
\centering\includegraphics[width=17cm]{Images/paperESODPh111.pdf}
\caption{
Here we reproduce the phase diagrams in a $[111]$ field as signalled  via the (a) Palmer-Chalker and (b) $\Gamma_{5}$ order parameters, as well as the quantity (c) $m_{6\phi}$ (defined below) to differentiate between $\psi_{2}$ and $\psi_{3}$ states. The contour of the phase diagram is clearly visible in panels (a) and (b). However, as explained in the main text, in order to understand the reentrance at $B\sim 0.5$ T, we need to consider the evolution of the angle $\phi$. The $\psi_{2}$ ($\psi_{3}$) states are characterized by $\phi \equiv n \pi/3\;(+\pi/6)$ for $n=0,...,5$. Hence, the quantity $m_{6\phi}\equiv m_{\Gamma 5} \cos\left(6\phi\right)$ is equal to +1 (-1) for $\psi_{2}$ ($\psi_{3}$) states. The yellow region at finite temperature for $B\sim 0.5$ T thus indicates the dominance of $\psi_{2}$ order in this region, as discussed in the main text.\\
All of these simulations were done for $L=6$ and $t_{m}=5. 10^{7}$ Monte-Carlo steps.
}
\label{fig:111SM}
\end{figure}
%------------------------------------------------------------------------


